Two-Sample Testing via Path-based Inference

Modern deep generative models are primarily studied for their ability to generate realistic samples, yet the generative dynamics they learn can also serve as objects of statistical inference. We develop this idea for two-sample testing, the problem of deciding whether the same distribution generated two finite datasets. Using stochastic interpolants, we connect both distributions to a shared Gaussian bottleneck, so that each half of the resulting path is a Gaussian channel acting on a single population. We prove that the null hypothesis holds if and only if the population denoiser, or equivalently, the velocity fields of the two halves, coincide at any single noise level, which amounts to a reflection symmetry of the path about the bottleneck. Deviations from this symmetry yield a continuum of two-sample witnesses, which we estimate via held-out regression risks on learned denoisers and velocities and aggregate along the path; under an information-theoretic weighting, the aggregated discrepancy equals the Jeffreys divergence between the noise-smoothed distributions. Calibrating the resulting statistics by permutation yields tests that are valid in finite samples for any trained networks and consistent when the fields are learned accurately. On a synthetic benchmark and three image benchmarks, the proposed tests improve power over the strongest baseline by up to 33 percentage points at an equal total sample budget, with the best choice of regression representation and path weighting depending on the data modality. These results show that generative paths provide a principled representation for statistical testing, extending stochastic-interpolant models beyond generation.

==> experiments/implementation_details.tex <==
\begin{table}[ht]
  \centering
  \caption{Dataset-specific configuration. (a)~Alternative, sample sizes and backbone;
    $\epsilon$ is the contamination fraction and, for HDGM, $0.5$ is the correlation of the
    first two coordinates under $\rho_1$. (b)~Optimisation settings and training time at the
    largest $n$, as mean $\pm$ standard deviation in minutes over five seeds and both
    representations (10 runs) on a single NVIDIA A100 GPU.}
  \label{tab:implementation-details}
  \small
  \textbf{(a) Data and model configuration}\\[2pt]
  \begin{adjustbox}{max width=\textwidth}
  \begin{tabular}{@{}lllll@{}}
    \toprule
    Dataset & Alternative & $n_{\mathrm{tr}}=n_{\mathrm{te}}$
      & Backbone & Backbone details \\
    \midrule
    HDGM
      & $d=10$, mean gap $0.5$, $corr.=0.5$
      & $500,1000,2000,4000$
      & FC-MLP
      & width 128, depth 4 \\
    MNIST
      & contamination $3\rightarrow8$, $\epsilon=0.1$
      & $50,100,150,180,200$
      & U-Net
      & $1\times28\times28$, $c=16$\\
    Fashion-MNIST
      & contamination $\textit{Sneaker}\rightarrow\textit{Ankle Boot}$, $\epsilon=0.1$
      & $50,100,150,180,200$
      & U-Net
      & $1\times28\times28$, $c=16$ \\
    OrganAMNIST
      & contamination $\textit{Left lung} \rightarrow \textit{Right lung}$, $\epsilon=0.1$
      & $100,200,350,420$
      & U-Net
      & $1\times64\times64$, $c=32$ \\
    \bottomrule
  \end{tabular}
  \end{adjustbox}

  \medskip
  \textbf{(b) Optimization and runtime}\\[2pt]
  \begin{adjustbox}{max width=\textwidth}
  \begin{tabular}{@{}lccccl@{}}
    \toprule
    Dataset & Batch size & Learning rate & Input normalisation
      & Recorded optimisation steps & Time at largest $n$ (min) \\
    \midrule
    HDGM & 1024 & $10^{-3}$ & no
      & $1300,1300,2600,5200$ & $1.56\pm0.47$ \\
    MNIST & 256 & $5\times10^{-4}$ & yes
      & 1600 & $0.86\pm0.02$ \\
    Fashion-MNIST & 256 & $5\times10^{-4}$ & yes
      & 2500 & $5.89\pm1.59$ \\
    OrganAMNIST & 256 & $5\times10^{-4}$ & yes
      & $1600,1600,3200,3200$ & $4.58\pm0.03$ \\
    \bottomrule
  \end{tabular}
  \end{adjustbox}
\end{table}
